Degrees-of-freedom penalized piecewise regression

Many popular piecewise regression models rely on minimizing a cost function on the model fit with a linear penalty on the number of segments. However, this penalty does not take into account varying complexities of the model functions on the segments potentially leading to overfitting when models with varying complexities, such as polynomials of different degrees, are used. In this work, we enhance on this approach by instead using a penalty on the sum of the degrees of freedom over all segments, called degrees-of-freedom penalized piecewise regression (DofPPR). We show that the solutions of the resulting minimization problem are unique for almost all input data in a least squares setting. We develop a fast algorithm which does not only compute a minimizer but also determines an optimal hyperparameter -- in the sense of rolling cross validation with the one standard error rule -- exactly. This eliminates manual hyperparameter selection. Our method supports optional user parameters for incorporating domain knowledge. We provide an open-source Python/Rust code for the piecewise polynomial least squares case which can be extended to further models. We demonstrate the practical utility through a simulation study and by applications to real data. A constrained variant of the proposed method gives state-of-the-art results in the Turing benchmark for unsupervised changepoint detection.

==> pseudocode/cv.tex <==
\begin{algorithmic}[1]
    \Input
        \State {Timeseries sample given by $(t_i)_{i=1,...,n}$, $(y_i)_{i=1,...,n}$}
        \State {User parameter: maximal total degrees of freedom $\nu_\text{max}^\text{tot}$}
        \State {Cut graph}
    \EndInput
    \Output
        \State {Function mapping penalties $\gamma$ to associated CV values}
    \EndOutput
    \State

    \State $\mathrm{CV} \gets~$ constant $0$ function

    \For{$r \in 1:n$} \Comment{For theoretical reasons might want to consider $2:n$ here instead}
        \State $\nu_{\max} \gets \min\{ \#(1:r), \nu_\text{max}^\text{tot} \}$
        \For{$\nu \in \texttt{reversed}(1:\nu_\text{max})$}
            \State $(P, \lambda) \gets~$ trace cut graph starting at $(r,\nu)$
            \State $\omega \gets~$ model corresponding to last segment of partition $P$
            \State $\mathrm{CV}_\nu \gets~$ error between $\omega(t_{r+1})$ and $y_{r+1}$
            \State $\text{error} \gets \sum_{I \in P} d_I^{\lambda(I)}$ \Comment{Model error of piecewise model}
            \State $\text{affine\_fn}_\nu \gets (\gamma \mapsto \nu \gamma + \text{error})$
        \EndFor
        \State Find pointwise minimum $f$ of $(\text{affine\_fn}_\nu)_{\nu}$
        \State $\mathrm{CV}_r^* \gets~$ piecewise constant function that equals $\mathrm{CV}_\nu$ at $\gamma$ whenever $f(\gamma) = \text{affine\_fn}_\nu(\gamma)$
        \State $\mathrm{CV} \gets \mathrm{CV} + \mathrm{CV}_r^*$
    \EndFor
    \State \Return $\gamma \mapsto \frac{\mathrm{CV}(\gamma)}{n}$ \Comment{Rescaling CV scores}
\end{algorithmic}

==> pseudocode/graph_tracing.tex <==
\begin{algorithmic}[1]
    \Input
        \State {Timeseries subsegment given by $(t_i)_{i=1,...,r}$, $(y_i)_{i=1,...,r}$}
        \State {Number of dofs $\nu$}
        \State {Cut graph $((B_r^\nu)_{r, \nu}$, $(\texttt{final\_cut}_r^\nu)_{r, \nu}$, $(\texttt{remaining\_dofs}_r^\nu)_{r, \nu})$}
    \EndInput
    \Output
        \State \parbox[t]{.9\linewidth}{Optimal partition $P \in \OPart(1:r)$ of subsegment $1:r$ and associated dof sequence $\lambda \in \Lambda(P)^\nu$}
    \EndOutput
    \Description
        \State \parbox[t]{.9\linewidth}{
            Get sequence of optimal cuts and associated remaining dofs by (transitively)
            following the edges in the cut graph starting at node $(r,\nu)$
            until reaching a node with no outgoing edges and recording each visited node.
        }
    \EndDescription
    \State


    \State cuts $~\gets~$ empty list
    \State $\lambda \gets~$ empty list

    % \State $(r_\text{curr}, \nu_\text{curr}) \gets (r, \nu)$ \Comment{Current node}

    \If{There is some cut $\texttt{final\_cut}_{r}^{\nu}$ in front of timeseries element $l+1$} % \Comment{Timeseries element after the final cut}
        \State {Add cut to cuts} \Comment{\parbox[t]{.5\linewidth}{Note that $l+1$ might be 1 which indicates a ``cut'' just in front of the segment}}
        \State $p_L \gets \texttt{remaining\_dofs}_{r}^{\nu}$ \Comment{Note that this is always strictly positive}
        \State $p_R \gets \nu - p_L$
        \State {Add $p_R$ to $\lambda$}
        \While {$p_L \geq 2$ and last added cut isn't in front of segment} % \Comment{\parbox[t]{.25\linewidth}{This loop is essentially an unrolled recursive call}}
            \If{There is some cut $\texttt{final\_cut}_{\text{l}}^{p_L}$ in front of timeseries element $l'+1$}
                \State {$p_L' \gets \texttt{remaining\_dofs}_{l}^{p_L}$}
                \State {$p_R' \gets p_L - p_L'$}
                \State{Add new cut to cuts and $p_R'$ to $\lambda$}
                \State $p_L \gets p_L'$ and $l+1 \gets l' + 1$
            \Else
                \State break
            \EndIf
        \EndWhile
        \State {Add last $p_L$ to $\lambda$}
        \State {Convert cuts into partition $P$}
    \Else
        \State {There are no cuts, hence $P$ contains just the full segment $1:r$ and $\lambda(1:r) = \nu$}
    \EndIf
    \State \Return {$P$ and $\lambda$}
\end{algorithmic}

==> pseudocode/main_fn.tex <==
\begin{algorithmic}
    \Function{DofPPR}{}\begin{varwidth}[t]{\linewidth}
        (\par
        \hskip\algorithmicindent \hspace{-7em} a timeseries sample given by $(t_i)_{i=1,...,n}$, $(y_i)_{i=1,...,n}$, \par
        \hskip\algorithmicindent \hspace{-7em} a model fitting function $\texttt{fit\_local\_model}(\text{timeseries segment}, \text{degrees of freedom})$,\par
        \hskip\algorithmicindent \hspace{-7em} user parameters (maximal total and local degrees of freedom $\nu_\text{max}^\text{tot}, \nu_\text{max}^\text{loc}$) \par
        \hspace{-\algorithmicindent - 4.5em})
    \end{varwidth}
    \For{relevant subsegment $I$ of timeseries} \Comment{Relevance depends on user parameters}
        \For{feasible degree of freedom $\nu$ on $I$} \Comment{feasible means $1 \leq \nu \leq \min\{\# I, \nu_\text{max}^\text{loc}\}$}
            \State $\omega \gets \texttt{fit\_local\_model}(t_I, y_I; \nu)$
            \State $d_I^\nu \gets \texttt{residual\_error}(\omega, t_I, y_I)$ \Comment{Calculate local residual error on segment}
        \EndFor
    \EndFor

    \State \texttt{solve\_dp}() \Comment{Obtain cut graph}
    \For{$\nu \in \texttt{reversed}(1:\nu_\text{max}^\text{loc}+1)$}
        \State \parbox[t]{.9\linewidth}{
            Get sequence of optimal cuts and associated remaining dofs by (transitively)
            following the edges in the cut graph starting at node $(n,\nu)$
            until reaching a node with no outgoing edges and recording each visited node.
        }
        \State \parbox[t]{.9\linewidth}{
            Convert the recorded information into a partition of the timeseries into discrete segments and determine the associated dofs for each segment -- so symbolically find $P \in \OPart(1:n)$ and $\lambda \in \Lambda(P)^\nu$.
        }
        \State $\text{error} \gets \sum_{I \in P} d_I^{\lambda(I)}$ \Comment{Model error of piecewise model}
        \State $\text{affine\_fn}_\nu \gets (\gamma \mapsto \nu \gamma + \text{error})$
    \EndFor

    \State Find pointwise minimum of $(\text{affine\_fn}_\nu)_{\nu}$ \Comment{This yields the \emph{model function}}
    \State Calculate CV scores \Comment{This yields the \emph{CV function}}

    \State \parbox[t]{.9\linewidth}{Select optimal (interval of) $\gamma$ based on desired criteria -- for example one standard error rule -- via CV function.}
    \State Determine associated optimal model via model function.
    \State \Return that model.
    \EndFunction
\end{algorithmic}


==> pseudocode/model.tex <==
\begin{algorithmic}
  \Input
  \State {Timeseries sample given by $(t_i)_{i=1,...,n}$, $(y_i)_{i=1,...,n}$}
  \State {User parameter: maximal total degrees of freedom $\nu_\text{max}^\text{tot}$}
  \State {Cut graph}
  \EndInput
  \Output
  \State {Function mapping penalties $\gamma$ to the solution of the $\gamma-$penalized problem~\ref{main:eq:proposed_model_intro}}
  \EndOutput
  \State

  \For{$\nu \in \texttt{reversed}(1:\nu_\text{max}^\text{tot}+1)$}
  \State $(P, \lambda) \gets~$ trace cut graph starting at $(n,\nu)$
  \State $\text{error} \gets \sum_{I \in P} d_I^{\lambda(I)}$ \Comment{Model error of piecewise model}
  \State $\text{affine\_fn}_\nu \gets (\gamma \mapsto \nu \gamma + \text{error})$
  \EndFor

  \State \Return pointwise minimum of $(\text{affine\_fn}_\nu)_{\nu}$
\end{algorithmic}

==> pseudocode/pointwise_min.tex <==
\begin{algorithmic}[1]
    \Input
        \State {Collection of affine functions \texttt{affines}}
    \EndInput
    \Output
        \State {Pointwise minimum of \texttt{affines}}
    \EndOutput
    \Require \parbox[t]{.9\linewidth}{\texttt{affines} strictly sorted by slope in descending order: \\ $\texttt{Slope}(\texttt{affines}_i) > \texttt{Slope}(\texttt{affines}_{i+1})~\forall i$}

    \Match{$\texttt{length}(\texttt{affines}$)}
        \Case{0}
            \State \Return $\textbf{Nothing}$ \Comment{No functions to minimize}
        \EndCase
        \Case{1}
            \State \Return A piecewise function consisting of the single affine function
        \EndCase
        \Case{otherwise}
            \State Initialize $\texttt{minimals}$ with the first two affine functions \Comment{In input order}
            \State Initialize $\texttt{jumps}$ with their intersection point \Comment{So the $x \in \R$ \st $g_1(x) = g_2(x)$}
            \For{each remaining affine function $\texttt{right\_fn}$}
                \State $\texttt{left\_fn} \gets$ last function in $\texttt{minimals}$
                \While{$\texttt{length}(\texttt{jumps}) \neq 0$ and $(\texttt{right\_fn} - \texttt{left\_fn})(\text{last point in }\texttt{jumps}) \leq 0$}
                    \State remove last elements from \texttt{minimals} and \texttt{jumps}
                    \State $\texttt{left\_fn} \gets$ new last function in $\texttt{minimals}$
                \EndWhile
                \State Compute the intersection point of \texttt{right\_fn} with the last function in \texttt{minimals}
                \State Add the new function and intersection point to the lists
            \EndFor
            \State \Return \parbox[t]{.9\linewidth}{A piecewise function defined by its $\texttt{jumps}$ and $\texttt{minimal}$ functions between those jump locations}
        \EndCase
    \EndMatch
\end{algorithmic}

==> pseudocode/solve_dp.tex <==
\begin{algorithmic}[1]
    \Input
        \State {Timeseries sample given by $(t_i)_{i=1,...,n}$, $(y_i)_{i=1,...,n}$}
        \State {User parameters (maximal total and local degrees of freedom $\nu_\text{max}^\text{tot}, \nu_\text{max}^\text{loc}$)}
    \EndInput
        \Output
        \State {The cut graph}
    \EndOutput
    \State

    \State $B_r^1 \gets d_{1:r}^1 \enskip \forall r \in 1:n$; \quad $B_r^0 \gets 0 \enskip \forall r \in 1:n$; \quad $B_0^\nu \gets 0 \enskip \forall \nu$ \Comment{Initialization for DP}
    \For{right segment boundary $r \in 1:n-1$}
        \For{total dof $\nu + 1 \in 2 : \min\{r + 1, \nu_\text{max}^\text{tot}\}$}
            \State $p_{R, \min}(l) \gets \max\{ 1, \nu + 1 - l\}$ \Comment{\parbox[t]{.5\linewidth}{We have to have $l > p_L$ so that there's enough datapoints in the right segment to ``spend'' all the dofs which is equivalent to this condition on $p_R$.}}
            \State $p_{R, \max}(l) \gets \min\{ r + 1 - l, \nu, \nu_\text{max}^\text{loc}\}$ \Comment{\parbox[t]{.45\linewidth}{$p_R \leq $ number of datapoints in segment $l:r$, and $p_R$ must not be larger than $\nu$ since at least $1$ dof has to be spent on $p_L$. It's further restricted by the maximal dof we allow on any segment.}}
            \State $\displaystyle (l^*, p_R^*) \gets \argmin_{\mathclap{\substack{l \in 0:r \\ p_R \in p_{R, \min}(l) : p_{R, \max}(l)}}} ~ B_l^{\nu - p_R} + d_{l+1:r+1}^{p_R}$
            \State $\displaystyle B_r^\nu \gets B_{l^*}^{\nu - p_R^*} + d_{l^*+1:r+1}^{p_R^*}$
            \If{whole segment $1:r+1$ is best approximated with a single model}
                \State $\texttt{final\_cut}_r^\nu \gets$ no final cut
                \State $\texttt{remaining\_dofs}_r^\nu \gets 0$ \Comment{Remaining dofs to be used on the left of the final cut}
            \Else
                \State $\texttt{final\_cut}_r^\nu \gets$ cut just in front of timeseries element $l^* + 1$ \Comment{$l^*$ might be $0$}
                \State $\texttt{remaining\_dofs}_r^\nu \gets p_L^* = \nu - p_R^*$
            \EndIf
        \EndFor
    \EndFor
    \State \parbox[t]{.9\linewidth}{
        We now have a graph with nodes $(r, \nu)$, for $r, \nu$ feasible as in the loops above.
        Each node has an associated value $B_r^\nu$, and there's an edge from $r,\nu$ to $r', \nu'$
        if there is a $\texttt{final\_cut}_r^\nu$ at $r'+1$ and $\texttt{remaining\_dofs}_r^\nu = r'$.
        We will call this the cut graph.
    }
    \State $\texttt{cut\_graph} \gets ((B_r^\nu)_{r, \nu}$, $(\texttt{final\_cut}_r^\nu)_{r, \nu}$, $(\texttt{remaining\_dofs}_r^\nu)_{r, \nu})$
    \State \Return $\texttt{cut\_graph}$
\end{algorithmic}


==> pseudocode/solve_dp_fn.tex <==
\begin{algorithmic}
    \Function{solve\_dp}{}()
    \State $B_r^1 \gets d_{1:r}^1 \enskip \forall r \in 1:n$; \quad $B_r^0 \gets 0 \enskip \forall r \in 1:n$; \quad $B_0^\nu \gets 0 \enskip \forall \nu$ \Comment{Initialization for DP}
    \For{right segment boundary $r \in 1:n-1$} \Comment{Compute Bellman values via DP}
        \For{total dof $\nu + 1 \in 2 : \min\{r + 1, \nu_\text{max}^\text{tot}\}$}
            \State $p_{R, \min}(l) \gets \max\{ 1, \nu + 1 - l\}$ \Comment{\parbox[t]{.5\linewidth}{We have to have $l > p_L$ so that there's enough datapoints in the right segment to ``spend'' all the dofs which is equivalent to this condition on $p_R$.}}
            \State $p_{R, \max}(l) \gets \min\{ r + 1 - l, \nu, \nu_\text{max}^\text{loc}\}$ \Comment{\parbox[t]{.45\linewidth}{$p_R \leq $ number of datapoints in segment $l:r$, and $p_R$ must not be larger than $\nu$ since at least $1$ dof has to be spent on $p_L$. It's further restricted by the maximal dof we allow on any segment.}}
            \State $\displaystyle (l^*, p_R^*) \gets \argmin_{\mathclap{\substack{l \in 0:r \\ p_R \in p_{R, \min}(l) : p_{R, \max}(l)}}} ~ B_l^{\nu - p_R} + d_{l+1:r+1}^{p_R}$
            \State $\displaystyle B_r^\nu \gets B_{l^*}^{\nu - p_R^*} + d_{l^*+1:r+1}^{p_R^*}$
            \If{whole segment $1:r+1$ is best approximated with a single model}
                \State $\texttt{final\_cut}_r^\nu \gets$ no final cut
                \State $\texttt{remaining\_dofs}_r^\nu \gets 0$ \Comment{Remaining dofs to be used on the left of the final cut}
            \Else
                \State $\texttt{final\_cut}_r^\nu \gets$ cut just in front of timeseries element $l^* + 1$
                \State $\texttt{remaining\_dofs}_r^\nu \gets p_L^* = \nu - p_R^*$
            \EndIf
        \EndFor
    \EndFor
    \State \parbox[t]{.9\linewidth}{
        We now have a graph with nodes $(r, \nu)$ -- for $r, \nu$ feasible as in the loops above.
        Each node has an associated value $B_r^\nu$, and there's an edge from $r,\nu$ to $r', \nu'$
        if there is a $\texttt{final\_cut}_r^\nu$ at $r'+1$ and $\texttt{remaining\_dofs}_r^\nu = r'$.
        We will call this the cut graph.
    }
    \State $\texttt{cut\_graph} \gets ((B_r^\nu)_{r, \nu}$, $(\texttt{final\_cut}_r^\nu)_{r, \nu}$, $(\texttt{remaining\_dofs}_r^\nu)_{r, \nu})$
    \State \Return $\texttt{cut\_graph}$
    \EndFunction
\end{algorithmic}

